Spatially resolved centrifugal magnetosphere caught in motion around the secondary component of $\rho$ Oph A

The recently discovered spectroscopic binary $\rho$ Oph A is a rare magnetic hot binary system composed of two early B-type stars, comprising a non-magnetic primary (Aa) and a slightly less massive magnetic secondary (Ab). Using near-IR interferometry, we aim to resolve the system's astrometric orbit. The high-spectral resolution VLTI/GRAVITY data also enables obtaining further information about the two stellar components, and about the centrifugal magnetosphere orbiting the magnetic star. We obtained a time-series of $K$-band interferometric data from VLTI/GRAVITY, and analyzed them with the geometrical model-fitting tool PMOIRED. The continuum was used to derive the relative astrometry and relative fluxes of the two components, leading to the astrometric orbital solution. Spectro-interferometry covering the Br$\gamma$ line was then used to obtain high-angular-resolution information about the dominant magnetospheric cloud in corotation with the magnetic Ab component. The combination of the astrometric orbital solution with the published radial velocities for both components led to a 3-dimensional orbital solution, dynamical masses, and a dynamical parallax, revealing a good agreement with previous estimates and confirming the previously inferred alignment of the orbital axis and the rotation axis of the Ab component, albeit at a much higher precision. Detailed analysis of the Br$\gamma$ spectrointerferometry then revealed the changing position of the magnetospheric cloud relative to the Ab component. Comparison to the location of the cloud predicted from $\rho$ Oph Ab's oblique rotator model and H$\alpha$ emission properties demonstrated excellent agreement. We are additionally able to demonstrate that the magnetic star exhibits prograde rotation. This represents the first time that the motion of a centrifugal magnetosphere has been detected in angularly resolved observations.

==> commented_text.tex <==
%Key points

%1) comparison to previous RV orbit (very similar, but more precise); note here also that the distance converges almost exactly to the Gaia parallax distance

%2) alignment of spin and orbital axes: $i_{\rm rot} = 73^{\circ+4}_{-6}$, $i_{\rm orb} = 71.31 \pm 0.07^\circ$: identical to within $2^\circ$, i.e.\ within uncertainty in $i_{\rm rot}$

%3) directional alignment of spin and orbit: Br$\gamma$ spectro-interferometry reveals that $\rho$\,Oph\,Ab is rotating in the same direction as it is orbiting. This is almost certainly expected if the stars were born from the same molecular cloud core, as they should have inherited the same same angular momentum vector. 

%4) magnetospheric astrometry: in a corotating magnetosphere, projected velocity should be a linear function of projected distance from the star. This is in fact precisely what is seen in the modeled position of the cloud. 

%5) Can the aligned rotational and orbital angular momentum vectors tell us anything about tidal evolution? formation conditions? or perhaps even be a clue to the asymmetry of the magnetosphere?


%Interferometric studies of the Be star Achernar determined the projection angle of the star's rotational axis on the sky. \citep{2014A&A...569A..10D} found that it is misaligned by about $30^\circ$, and that the orbit and rotation are in the same direction (counter-clockwise on the sky) \citep{2022A&A...667A.111K} 

%\cite{2025A&A...694A.208K} found prograde disk rotation in the Be-sdO binary HD\,6819 using VLTI/GRAVITY interferometry. \textbf{Presumably other stars?} \RKl{HR~2142 also using GRAVITY \citep{2024ApJ...962...70K}}

%\cite{2024MNRAS.527.3982L} reported possible prograde rotation from the eclipsing contact binary ASAS J082243+1927.0, based on spot longitude. 

%\cite{2015MNRAS.448..429B} used spot rotation in {\em Kepler} eclipsing binaries to demonstrate retrograde and prograde rotation. 

%\cite{2022PASP..134h2001A} provide an overview of spin-orbit obliquity and prograde/retrograde orbits in exoplanetary systems. This is possible using the starspot tracking method. 

%\cite{2023A&A...678A.204S}: Survival of fossil fields during the pre-main sequence evolution of intermediate-mass stars. Field survivability during protostellar phase linked to transition to radiative, set by accretion rate: lower accretion rate means a stronger field; higher resistivity leads to more rapid field decay; 

%\cite{2018MNRAS.481.2450W}: On the origin of magnetic fields in stars

%\cite{2022MNRAS.511..746W}: effect of high-resolution (kG fields are possible)

%\subsection{Is spin-orbit alignment a clue to magnetospheric asymmetry?}

%In general the magnetospheres of stars with tilted dipoles should be symmetric about reflection along the rotational and magnetic axes. For a tilted dipole, the expected circumstellar plasma distribution is two clouds of equal size on either side of the star, located at the intersections of the magnetic and equatorial planes, with the clouds oriented approximately perpendicularly to the magnetic axis. A non-dipolar magnetic field can of course introduce some degree of asymmetry, as in the case of $\sigma$\,Ori\,E, but $\rho$\,Oph\,A's magnetic field does not depart strongly from a dipole, despite its asymmetry being so pronounced that the second cloud is almost undetectable. 

%Only two other stars have been observed with comparable magnetospheric asymmetry to $\rho$\,Oph\,Ab's, both of which are magnetic binaries: HD\,156324 and HD\,37017. HD\,156324 is a closely bound ($P_{\rm orb} \sim 1.5$~d) tidally locked binary, and its dominant magnetospheric cloud appears to be located at the Lagrange L2 point. HD\,37017 is more similar to $\rho$\,Oph, in that its 30~d orbit is fairly eccentric, and it is not tidally locked. 

%Notes: 

%\begin{figure}
%\begin{center}
%\includegraphics[width=0.5\textwidth]{effective_rk.pdf}
%\end{center}
%\caption[]{Schematic illustrating the variation in the effective Kepler radius with longitude. We are looking down at the star, which is rotating counter-clockwise. The direction of the orbit is from right to left, and side facing the primary is towards the bottom. The Kepler radius for the non-orbiting, single-star case is shown by the solid blue circle; the dashed blue circle shows the outermost extent of H$\alpha$ emission. The solid and dashed red ovals show the effective Kepler radius at periastron and apastron, respectively.}
%\label{fig:effective_rk}
%\end{figure}


%Lagrange L1 and L2 points are a minimum of about 0.3 AU from the secondary (at periastron), about 21 stellar radii. This is well outside both the H$\alpha$ magnetosphere (maximum extent about 4.5 $R_*$) and the Alfv\'en radius (about 10 $R_*$). It seems unlikely the Lagrange points have any effect on the magnetosphere. 

%Orbital motion will make a contribution to the magnetospheric velocity fields. The orbital velocity varies between about 100 and 150 \kms~between apastron and periastron. The densest points in the magnetosphere are at the Kepler corotation radius $R_{\rm K} = 1.9\,R_*$, at the intersections of the rotational and magnetic equatorial planes. The rotational velocity at $R_{\rk K}$ should therefore be about 430 \kms. Given prograde rotation, the orbital velocity will add to the rotational velocity when the magnetosphere is on the side of the star directly opposite the primary, and will subtract from the rotational velocity when the magnetosphere is on the side facing the primary, thus the net velocity at $R_{\rm K}$ will vary between 280 and 580 \kms. In principle this should mean that the magnetospheric plasma is subjected to stronger rotational support when it is on the opposite side from the primary, and weaker rotational support when it is between the primary and the secondary. In principle this should cause the value of $R_{\rm K}$ to vary with longitude: at periastron, the effective Kepler radius on the side opposite the primary should be about 1.5 $R_*$, while on the side facing the primary it should be about 4 $R_*$. This variation in the effective Kepler radius could make it easier for material to leak out of the magnetosphere on the inward facing side. 

%The next question is whether, if the effective Kepler radius moves above a given parcel of matter, it will have sufficient time to fall back to the star before the effective Kepler radius returns to its initial position. Taking a parcel of material at the nominal (non-orbiting) Kepler radius, the gravitational free-fall timescale is approximately 8700 sec or about 13\% of the rotational period. Since the material exactly at $R_{\rm K}$ will spend half a rotational cycle below the effective Kepler radius, there should be sufficient time for the innermost material to drain towards the star. Material close to the outer radius of emission, however, has a free-fall timescale of about half a rotational cycle, and will therefore remain inside the centrifugal magnetosphere despite the change in effective Kepler radius. 

%We see that the gravitocentrifugal potential should be modified by the the centrifugal contribution of the orbital motion, and that this can plausibly affect the plasma distribution in the magnetosphere. However, the two clouds should be located at symmetrical positions on either side of the star, with their central positions within the orbital and rotational planes at all rotational phases, and should therefore be subjected to the same net combination of forces as the star rotates. In order to break the symmetry, one of the clouds would have to be subjected to a net difference in force as compared to the other cloud. 

%If there was a harmonic relationship between the orbital and rotational periods, such that one side was more often facing the primary at periastron, this could lead to an asymmetric plasma distribution over time. However, the ratio of the orbital to the rotational period is close to (but not precisely) 117.5:1, meaning that neither magnetic hemisphere should be preferentially subjected to stronger rotational support at periastron. 

%Another possibility is some asymmetry in the magnetic field itself. However, the \bz~curve shows no sign of significant departures from a magnetic dipole. 

%We conclude that while there are almost certainly important modifications to the gravitocentrifugal potential due to orbital motion, the orbital properties of the system do not show any obvious means of breaking the expected magnetospheric symmetry. 

%Possible dynamical/tidal effects: 

%1) Lagrange points: these are too far away to make much difference
%2) preferential orientation at periastron: if one side of the star is more often facing the primary at periastron than the other, this could introduce a slight gravitational preference for material to accumulate on one side; however, there is no obvious orbital harmonic, with the ratio of the orbital to rotational periods being closed to, but not exactly, 117.5. Even if it was {\em exactly} 235:2, this would mean alternate sides of the star facing the primary on alternating orbital cycles, i.e.\ no net preference.
%3) contribution of the centrifugal force of the orbit to the gravitocentrifugal potential: given the prograde rotation of the star, on the inward-facing side the net velocity of the plasma is slightly reduced (since the orbital and rotational vectors are in opposition), while on the side facing away they are slightly enhanced (the vectors are in the same direction). However, if the rotational axis is indeed exactly aligned with the orbital axis, both magnetospheric clouds should experience the same net combination of forces throughout a rotational cycle. If the rotational axis is slightly tilted, however, such that the angle between the magnetic equatorial plane and the orbital plane changes throughout a rotational cycle, there could be some effect, as this would lead to one of the clouds receiving a stronger contribution from the centrifugal influence of the orbit. 
